A Traffic Management Framework for On-Demand Urban Air Mobility Systems

Urban Air Mobility (UAM) offers a solution to current traffic congestion by providing on-demand air mobility in urban areas. Effective traffic management is crucial for efficient operation of UAM systems, especially for high-demand scenarios. In this paper, we present a centralized traffic management framework for on-demand UAM systems. Specifically, we provide a scheduling policy, called VertiSync, which schedules the aircraft for either servicing trip requests or rebalancing in the system subject to aircraft safety margins and energy requirements. We characterize the system-level throughput of VertiSync, which determines the demand threshold at which passenger waiting times transition from being stabilized to being increasing over time. We show that the proposed policy is able to maximize throughput for sufficiently large fleet sizes. We demonstrate the performance of VertiSync through a case study for the city of Los Angeles, and show that it significantly reduces passenger waiting times compared to a first-come first-serve scheduling policy.

==> proof-renewal-sufficient-2.tex <==
\section{Proof of Theorem \ref{thm:renewal-sufficient-2}}\label{section:proof-renewal-sufficient-2}
We follow the same line of proof as in Theorem~\ref{thm:renewal-sufficient}. For brevity, we only highlight the major differences.

At the start of the $(k+1)$-th cycle, we solve the LP \eqref{eq:linear-program} and we let $K_{i}^{*}$, $i \in [\numsafesch]$, be its solution. We then construct a feasible solution to the optimization problem \eqref{eq:TFMP-objective}-\eqref{eq:TFMP-energy-constraints} as follows:
\begin{enumerate} 
\item choose a service vector $\routingvec{}{i} \in \safeschset$ with $K_{i}^{*} > 0$, and, before activating $\routingvec{}{i}$, distribute the aircraft in the system so that for any $p \in \routeset$ with $\routingvec{p}{i} > 0$, there is
    \begin{equation*}
       \aircraftcard_p := \frac{\routingvec{p}{i}}{\sum_{p \in \routeset}\routingvec{p}{i}}\aircraftcard 
    \end{equation*}
    aircraft at vertiport $o_p$. The initial distribution of aircraft takes at most $\aircraftcard \overline{T}$ minutes.
\item once the initial distribution is completed and the airspace is empty, activate $\routingvec{}{i}$ for a duration of 
\begin{equation*}
    \max_{p \in \routeset: \routingvec{p}{i} > 0} \frac{\aircraftcard_p}{\routingvec{p}{i}}\cruisetau
\end{equation*}
minutes. At the end of this interval, $\aircraftcard_p$ trips (out of $\Queuelength{p}(t_{k+1})$) will be serviced for all $p \in \routeset$. 
\item Once step 2 is completed and the airspace is empty, we re-balance the aircraft using $\routingvec{}{i}$'s ``reversed" service vector, i.e., a service vector $\routingvec{}{j} \in \safeschset$ such that for all $p \in \routeset$ with $\routingvec{p}{i} > 0$, $\routingvec{q}{j} = \routingvec{p}{i}$, where $q = (d_p,o_p)$ is the opposite O-D pair to the pair $p$. It takes at most $\overline{T}$ minutes for the airspace to become empty, and an additional $\lceil E_{p}/E_{\text{inc}}\rceil \cruisetau$ recharging time before the first aircraft is ready for rebalancing. Therefore, the rebalancing process takes at most
\begin{equation*}
        \max_{p \in \routeset: \routingvec{p}{i} > 0} \left(\frac{\aircraftcard_p}{\routingvec{p}{i}} + \lceil\frac{E_{p}}{E_{\text{inc}}}\rceil \right)\cruisetau + \overline{T}
\end{equation*} 
minutes. 
\item Repeat steps 1 to 3 until the service vector is used for a total duration of $(K_{i}^{*}+1)\cruisetau$ minutes. This will take at most 
\begin{equation*}
    N_p := \left\lceil \frac{\routingvec{p}{i} K_i^{*}}{\aircraftcard_p} \right\rceil + \left\lfloor \frac{\routingvec{p}{i} K_i^{*}}{\aircraftcard_p} \right\rfloor 
\end{equation*}
number of iterations. Therefore, steps 1 to 3 are repeated for a total duration of  
\begin{equation*}
     \max_{p \in \routeset: \routingvec{p}{i} > 0} (\left(\frac{\aircraftcard_p}{\routingvec{p}{i}} + \lceil\frac{E_{p}}{E_{\text{inc}}}\rceil \right)\cruisetau + \overline{T})N_p
\end{equation*}
minutes. At the end of this time interval, $\routingvec{p}{i} K_i^{*}$ trips will be serviced for all $p \in \routeset$.
\item Repeat steps 1 to 3 for another service vector in $\safeschset$. Once these steps are completed for every service vector $\routingvec{}{i} \in \safeschset$ with $K_{i}^{*} > 0$, $\sum_{i=1}^{\numsafesch}\routingvec{p}{i}K_{i}^{*}$ requests will be serviced for each O-D pair $p \in \routeset$. From the constraint of the LP \eqref{eq:linear-program}, it follows that all the requests for the $(k+1)$-th cycle will be serviced and the cycle ends.
\end{enumerate}
By combining all the above steps, it follows that
\begin{equation}\label{eq:cycle-upper-bound-2}
\begin{aligned}
        \Cyclelength(k+1) &\leq \sum_{i=1}^{\numsafesch}\max_{p \in \routeset: \routingvec{p}{i} > 0} (\left(\frac{\aircraftcard_p}{\routingvec{p}{i}} + \lceil\frac{E_{p}}{E_{\text{inc}}}\rceil \right)\cruisetau + \overline{T})N_p \\
        &\leq 2\sum_{i=1}^{\numsafesch} K_i^{*} + \sum_{i=1}^{\numsafesch} 2\frac{\sum_{p \in \routeset}\routingvec{p}{i}}{\aircraftcard}C K_{i}^{*},
\end{aligned}
\end{equation}

